Bullseye Polytope: A Scalable Clean-Label Poisoning Attack with Improved Transferability

A recent source of concern for the security of neural networks is the emergence of clean-label dataset poisoning attacks, wherein correctly labeled poison samples are injected into the training dataset. While these poison samples look legitimate to the human observer, they contain malicious characteristics that trigger a targeted misclassification during inference. We propose a scalable and transferable clean-label poisoning attack against transfer learning, which creates poison images with their center close to the target image in the feature space. Our attack, Bullseye Polytope, improves the attack success rate of the current state-of-the-art by 26.75% in end-to-end transfer learning, while increasing attack speed by a factor of 12. We further extend Bullseye Polytope to a more practical attack model by including multiple images of the same object (e.g., from different angles) when crafting the poison samples. We demonstrate that this extension improves attack transferability by over 16% to unseen images (of the same object) without using extra poison samples.

==> appx-diff-coeffs-single-target-attack-acc.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/diff-coeffs/DPN92-attack-acc-avg.pdf}
         \caption{\scriptsize DPN92}
         \label{fig:apx-diffcoeffs-single-tr-DPN92}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/diff-coeffs/SENet18-attack-acc-avg.pdf}
         \caption{\scriptsize SENet18}
         \label{fig:apx-diffcoeffs-single-tr-SENet18}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/diff-coeffs/ResNet50-attack-acc-avg.pdf}
         \caption{\scriptsize ResNet50}
         \label{fig:apx-diffcoeffs-single-tr-ResNet50}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/diff-coeffs/ResNeXt29_2x64d-attack-acc-avg.pdf}
         \caption{\scriptsize ResNeXt29\_2x64d}
         \label{fig:apx-diffcoeffs-single-tr-ResNeXt29_2x64d}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/diff-coeffs/GoogLeNet-attack-acc-avg.pdf}
         \caption{\scriptsize GoogLeNet}
         \label{fig:apx-diffcoeffs-single-tr-GoogLeNet}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/diff-coeffs/MobileNetV2-attack-acc-avg.pdf}
         \caption{\scriptsize MobileNetV2}
         \label{fig:apx-diffcoeffs-single-tr-MobileNetV2}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/diff-coeffs/ResNet18-attack-acc-avg.pdf}
         \caption{\scriptsize ResNet18}
         \label{fig:apx-diffcoeffs-single-tr-ResNet18}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/diff-coeffs/DenseNet121-attack-acc-avg.pdf}
         \caption{\scriptsize DenseNet121}
         \label{fig:apx-diffcoeffs-single-tr-DenseNet121}
     \end{subfigure}
     \caption{Linear transfer learning: Success rates of BP and the other nine alternatives depicted at Figure~\ref{fig:examples}, against each individual victim model.}
     \label{fig:apx-diffcoeffs-single-tr-individualVictim}
\end{figure*}

==> appx-single-target-attack-acc.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/single-target/transfer/DPN92-attack-acc-avg.pdf}
         \caption{\scriptsize DPN92}
         \label{fig:single-tr-DPN92}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/single-target/transfer/SENet18-attack-acc-avg.pdf}
         \caption{\scriptsize SENet18}
         \label{fig:single-tr-SENet18}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/single-target/transfer/ResNet50-attack-acc-avg.pdf}
         \caption{\scriptsize ResNet50}
         \label{fig:single-tr-ResNet50}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/single-target/transfer/ResNeXt29_2x64d-attack-acc-avg.pdf}
         \caption{\scriptsize ResNeXt29\_2x64d}
         \label{fig:single-tr-ResNeXt29_2x64d}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/single-target/transfer/GoogLeNet-attack-acc-avg.pdf}
         \caption{\scriptsize GoogLeNet}
         \label{fig:single-tr-GoogLeNet}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/single-target/transfer/MobileNetV2-attack-acc-avg.pdf}
         \caption{\scriptsize MobileNetV2}
         \label{fig:single-tr-MobileNetV2}
     \end{subfigure}
     
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/single-target/transfer/ResNet18-attack-acc-avg.pdf}
         \caption{\scriptsize ResNet18}
         \label{fig:single-tr-ResNet18}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/single-target/transfer/DenseNet121-attack-acc-avg.pdf}
         \caption{\scriptsize DenseNet121}
         \label{fig:single-tr-DenseNet121}
     \end{subfigure}
     \caption{Linear transfer learning: Success rates of CP, \sysshortOne{}, \sysshortThree{} and \sysshortFive{}, against each individual victim model.}
     \label{fig:single-tr-individualVictim}
\end{figure*}

==> bp-alts-example-5.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.17\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth, frame]{images/examples/1.pdf}
         \label{fig:example-1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.17\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth, frame]{images/examples/2.pdf}
         \label{fig:example-2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.17\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth, frame]{images/examples/4.pdf}
         \label{fig:example-4}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.17\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth, frame]{images/examples/7.pdf}
         \label{fig:example-7}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.17\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth, frame]{images/examples/10.pdf}
         \label{fig:example-10}
     \end{subfigure}
     \caption{Four alternatives of \sys{} with different sets of nonuniform coefficients. The blue circles are poisons with their coefficients displayed next to them, and the red cross is the target. Entropy of the coefficients increases from left to right. Note that the right most picture represents \sysshortOne{}.
     %We evaluate \sysshortOne{} against these nine alternatives in the linear transfer learning setting to measure the effectiveness of putting the target at the center of the poisons' polytope.
     }
\label{fig:5examples}
\end{figure*}

==> impact.tex <==
Compared to other types of data poisoning attacks, clean-label poisoning attacks are applicable in more realistic scenarios, as the poisoned data (1) will not be identified by human observers, and (2) does not degrade test accuracy on non-targeted objects, and therefore is not revealed until inference time.
To the best of our knowledge, a defense has not yet been proposed for this class of attacks.
When evaluating the state-of-the-art of such attacks, Convex Polytope, we found it to be very slow, taking an average of 17 hours to craft poisons for a single target.
This means that collecting statistics for just 50 different targets for a single set of hyperparameters requires 850 computational hours
(note that we use state-of-the-art \texttt{NVIDIA Titan RTX} Graphics cards in our experiments).
Unfortunately, this can be a barrier for high-impact research in this area, as it is simply impossible to gather the necessary data for thorough statistical evaluation.
In this work, we propose \sys{}, which is from the same family as Convex Polytope.
\sys{} not only beats Convex Polytope considerably, it is also an order of magnitude faster. 
When building on previous results, e.g., for designing defenses, being able to run the attack in a short time makes a huge difference.
In this light, our work will stimulate future research by severely cutting down computing time.

Furthermore, the intuition behind \sys{} is strongly supported by our numerical results, and indicates a promising direction for improving the robustness of attacks in general.
While the geometric mean of feature vectors is taken as a heuristic estimate of the ideal center point (that has the max-min optimum distance from the polytope’s sides), it may not always be close to the ideal ``deepest point.'' Finding this ideal point is shown to be intractable when we do not have access to the bounding planes of the polytope (which is our case), but further analysis and experimentation may yield better heuristics to approximate it.
While our work provides plausible intuition backed by experiments, searching for theoretical guarantees may provide deeper insight that further improves attack accuracy and robustness. 

